BarQL: Collaborating Through Change

Applications such as Google Docs, Office 365, and Dropbox show a growing trend towards incorporating multi-user live collaboration functionality into web applications. These collaborative applications share a need to efficiently express shared state, and a common strategy for doing so is a shared log abstraction. Extensive research efforts on log abstractions by the database, programming languages, and distributed systems communities have identified a variety of optimization techniques based on the algebraic properties of updates (i.e., pairwise commutativity, subsumption, and idempotence). Although these techniques have been applied to specific applications and use-cases, to the best of our knowledge, no attempt has been made to create a general framework for such optimizations in the context of a non-trivial update language. In this paper, we introduce mutation languages, a low-level framework for reasoning about the algebraic properties of state updates, or mutations. We define BarQL, a general purpose state-update language, and show how mutation languages allow us to reason about the algebraic properties of updates expressed in BarQ L .

==> incremental.tex <==
\section{Incremental Rewrite Selection}
\label{sec:inc}

The time complexity of the deletion and rewrite oracles defined in Section \ref{sec:reduction:barqloracle} is unbounded.  As such
they are not practice definitions to formalize an implementation. 
Furthermore, for a log of size $n$, after every insertion there are $O(n)$ deletion candidates, and $O(n^2)$ rewrite candidates.  
Once again, this is impractical for any realistic implementation.  In this section we provide definitions for incremental
rewrites. Our goal is to provide a formalism that is {\em close} to a realistic implementation. Thus, our formalism can
serve as a system specification for future implementations. 

\begin{definition}
An incremental log rewrite oracle $\mathcal O_R$ for rewrite classes $R$ maintains metadata $\mu_i$ for every log state $i$ such that:
$$\mathcal O_R(\mu_n, \mut_{n+1}) = \tuple{\mu_{n+1}, \{r_1, r_2, \ldots\}}$$
where $r_1, r_2, \ldots$ is the set of all rewrites $r_j \in R$, which are both correct and recoverable for log $\mut_1,\ldots,\mut_{n+1}$, but not for log $\mut_1,\ldots,\mut_n$.
\end{definition}

We now construct an incremental log rewrite oracle $\mathcal O_R$ for $R = \{deletion,composition\}$.

\subsection{Incremental Deletion Rewrites}
%We first consider an incremental version of the subsumption oracle for hierarchical collections.  
%Concretely, we are looking for an operation $\oraclesub_\Delta : \mut \times \mu \mapsto {\bf bool} \times \mu$ such that
%$$\oraclesub_\Delta(\mut', \mu_\mut) = \tuple{\oraclesub(\mut, \mut'), \mu'}$$
%$$\oraclesub_\Delta(\mut'', \mu') = \tuple{\oraclesub(\mut, \mut' \circ \mut''), \mu''}$$

The {\em unsubsumed fragment} $\mut_{\oraclesub,\mathbb M}$ of a composite mutation $\mut$  with respect to a list of composite mutations $\mathbb M$ is the set of mappings 

$$\mut_{\oraclesub,\mathbb M} := \condset{\tuple{\phi \mapsto \mut(\phi)}}{\begin{array}{l}
\phi \in \mut \wedge \not\exists i,\phi' \in \mathbb M_i : \\
\ \ \ \ (\phi' \subset \phi \wedge S(M'(\phi'))) \vee\\
\ \ \ \ (\phi' = \phi \wedge S(M(\phi), M'(\phi)))
\end{array}}$$

\begin{lemma}
For mutations with bounded path lengths, the unsubsumed fragment of a mutation of bounded complexity can be maintained incrementally for the addition of a mutation of bounded complexity to $\mathbb M$ in constant time.
\end{lemma}

\proof{Incremental maintenance requires a bounded number of existential quantifications over sets of bounded size, and a like number of invocations of the subsumption oracle}.

\tinysection{The Subsumption Index}
A subsumption index is a datastructure constructed for a log of mutations in $\collbar$ with bounded path length and complexity.  For each mutation $\mut_x$ in the log, the subsumption index maintains the unsubsumed fragment of $\mut_x$ with respect to mutations $\mut_{x+1} \ldots \mut_n$, where $n$ is the length of the log.  The subsumption index maintains a hash-map from each path $\phi$ to a bi-directionally linked-list of pointers to each unsubsumed fragment containing a mapping from $\phi$ or one of its descendents $\phi' \subset \phi$.  We refer to these linked lists as the {\em target lists} of the index.  For each unsubsumed fragment, the subsumption index maintains a list of pointers to each target list entry pointing to it.

\begin{lemma}
\label{lem:subsumptionidempotent}
The subsumption oracle for simple mutations in $\collbar$ is true iff the subsuming mutation is idempotent.
\end{lemma}

\proof{By the definition of the subsumption oracles for simple mutations and $\lbar$}

\smallskip

\begin{lemma}
\label{lem:subsumptionindexcomplexity}
The amortized incremental processing cost of incrementally maintaining a subsumption index is constant for each insertion.
\end{lemma}

\proof{The cost of inserting (resp. deleting) a mutation into (resp. from) a subsumption index's hash map is constant if the mutation has bounded path length and complexity

By Lemma \ref{lem:subsumptionidempotent}, the idempotence of a simple mutation $M$ is equivalent to $M$ subsuming any simple mutation.  Testing idempotence for all simple mutations in a composite mutation $M \in \mut$ where $\mut$ is of bounded complexity, can be done in constant time.  

For each of the (constant number of) paths $\phi \in \mut$ that maps to an idempotent simple mutation, the index provides a constant time lookup of all mutations that $\mut(\phi)$ subsumes.  For a mutation with bounded complexity and path length, there are a bounded number of target lists that could be subsumed.  

The cost of iterating over each target list (to update each unsubsumed fragment contained with in) can be amortized by attributing each update to the original insertion into the log of each mutation appearing in the target list.}

\begin{lemma}
\label{lem:readrestrictions}
If $\mut \sqcup \readset(\mathbb M_1\circ\ldots\circ\mathbb M_n) = \emptyset$ then all elements of $\mut \sqcup \readset(\mathbb M_1\circ\ldots\circ\mathbb M_n \circ \mut')$ must appear in the unsubsumed fragment $\mut_{\oraclesub,\mathbb M}$
\end{lemma}

\proof{By Algorithm \ref{alg:compose}, an element of the read path of $\mut'$ can only appear in the read set of $\mathbb M_1\circ\ldots\circ\mathbb M_n\circ \mut'$ if it appears in the read set of $\mathbb M_1\circ\ldots\circ\mathbb M_n$, or appears in none of the mutations $\mathbb M_1, \ldots, \mathbb M_n$.  }

\smallskip

If $\oraclesub$ is the subsumption oracle for $\collbar$, then by the definition of unsubsumed fragments and Lemma \ref{lem:readrestrictions}, and the necessary conditions for $\oraclesub(\mut, (\mathbb M_1\circ\ldots\circ\mathbb M_n))$ become:
\[
\begin{array}{lcr}
\not \exists i : \mut \sqcup (\readset(\mathbb M_i) - \bigcup_{1 \leq j < i} \mathbb M_j) & \ \ &
\mut_{\oraclesub,\mathbb M} = \emptyset
\end{array}
\]

If the read set of any mutation $\readset{\mathbb M_i}$ in the log contains an ancestor or descendent of a mutation in the unsubsumed fragment of $\mut$ up through log entry $i$, $\mut$ can not be deleted until $\readset(\mathbb M_i)$ is deleted, or unless the overlapping path is removed from its read set.  We refer to this as a read conflict.

\tinysection{Read Blocks} 
We now introduce a new concept into the subsumption index datastructure.  In addition to containing pointers to unsubsumed fragments, a target list may also contain {\em read blocks}.  When a read conflict is detected, we insert a read block into all conflicting paths.  When iterating over a target list to update the unsubsumed fragments that it points to, only fragments corresponding to updates more recent than the read block are updated.  The subsumption index maintains a list of pointers from each mutation in the log to all read blocks created by that mutation.  

\smallskip

Each read block maintains a ready indicator: a boolean value initialized to false.  When iterating over a target list, the ready indicator of the first read block is set.  If and when the read block is removed, if its ready indicator has been set, the update iteration is continued.

\begin{lemma}
\label{lem:readblockchangefree}
The amortized cost of updating each unsubsumed fragment in a target list is unaffected by the presence of one or more a read block.
\end{lemma}

\proof{Scanning over target list entries more recent than the read block can be performed without touching unaffected entries, and only the first read block encountered need be touched.  The fixed cost of continuing an iteration can be attributed to the deletion of the read block, while the remaining cost is unchanged, and continues to be attributed to the insertion of the unsubsumed fragment being updated.}

\begin{theorem}
Given a log of mutations in $\collbar$, the set of log entries that can be deleted due to the insertion of a new update can be determined incrementally in amortized constant time, if log entries have bounded complexity and path length.
\end{theorem}

\proof{By maintaining the last index to output a new value of each path $\phi$ alongside the target lists, we can evaluate $(\readset(\mut) - \bigcup_{i} \mathbb M_i)$ in constant time for mutations of bounded complexity and path length.  Thus the cost of identifying and inserting any necessary read blocks is a constant.

By Lemmas \ref{lem:subsumptionindexcomplexity} and \ref{lem:readblockchangefree}, the remaining costs of maintaining and applying the subsumption index are amortized constant.}

\subsection{Incremental Composition Rewrites}

\begin{lemma}
\label{lem:commutativitytransitive}
Excluding the $\idmut$ mutation, commutativity of all other simple mutations in $\collbar$ is transitive.
\end{lemma}

\proof{Excluding $\idmut$, there are 4 types of simple mutation $M \in \collbar$: $\emptyset$ and $\Null$ from $\coll\mutlang$ only commute with mutations of the same type, destructive mutations $Q$ never commute, and update mutations $\tuple{\theta, Q}$ only commute with other update mutations with the same $\theta$.}

\tinysection{The Commutativity Index}
A commutativity index is a datastructure constructed for a log $\mathbb M$ of composite mutations in $\collbar$ with bounded path length and complexity.  The index consists of three hash-maps.  The index map maps each path $\phi$ to the 5-tuple $\tuple{start, op, end, child, read}$.  $start$ is the highest log index such that $\mathbb M_{start}(\phi) \neq \idmut$.  $op \in (\{destructive, \emptyset, \Null\} \cup \theta)$ is the {\em operation class} corresponding to simple mutation $\mathbb M_{start}(\phi)$.  If $op = destructive$ then $end = start$, otherwise $end$ is the highest log index such that $\mathbb M_{end}(\phi) \neq \idmut$ and $\mathbb M_{end}(\phi)$ does not correspond to $op$.  $child$ is the highest value of $start$ for a descendent of $\phi$.  $read$ is the highest log index such that $\phi \sqsubseteq \readset(\mathbb M_{read})$.

The remaining two hash-maps are similar to the map of target lists in the subsumption index.  The first maps paths to mutations in which the path appears, while the other maps paths to mutations for which the path appears in the mutation's read set.  We refer to these maps as the write and read deletion maps (respectively).

\begin{lemma}
A commutativity index can be incrementally maintained in $O(|\readset(\mut)|)$ time for an insertion of a mutation $\mut \in \collbar$ of bounded path length and complexity, into the log.
\end{lemma}

\proof{Inserting a composite mutation with bounded path length and complexity into the log requires a bounded number of modifications to the index and write deletion maps, and $O(|\readset(\mut)|)$ modifications to the read deletion map.}


\begin{lemma}
\label{lem:hierarchicalcommutativity1}
Given a commutativity index built over a sequence of composite mutations $\mathbb M$, for any composite mutation $\mut \in \collbar$ of bounded path length and complexity, the highest log index $i$ for which $\mathbb M_i \sqcap \mut \neq \emptyset$ can be computed in constant time.
\end{lemma}

\proof{The index $i$ is the maximum of the $child$ values for all paths $\phi \in\mut$, and all $start$ values for parents of paths $\phi\in\mut$.}

\begin{lemma}
\label{lem:hierarchicalcommutativity2-1}
Given a commutativity index built over a sequence of composite mutations $\mathbb M$, for any composite mutation $\mut \in \collbar$ of bounded path length and complexity, the highest log index $i$ for which there exists a path such that $\neg C(\mathbb M_i(\phi), \mut(\phi))$ can be computed in constant time.
\end{lemma}

\proof{For any path $\phi$, either $\mut(\phi) = \idmut$ and commutes with everything, $\mut(\phi)$ is destructive and commutes with nothing, or $\mut(\phi)$ commutes only with members of the same operation class.  In each case, the maximal index for the path is immediately evident or can be computed from $start$, $op$, and $end$.  The index $i$ is the maximal index for all paths.}

\begin{lemma}
\label{lem:hierarchicalcommutativity2-2}
Given a commutativity index built over a sequence of composite mutations $\mathbb M$, for any composite mutation $\mut \in \collbar$ of bounded path length and complexity, the highest log index $i$ for which $\mathbb M_i$ commutes with all subsequent log entries can be determined in constant time.
\end{lemma}

\proof{By Lemma \ref{lem:hierarchicalcommutativity2-1}, we can identify all mutations that commute with the tail of the log.  By transitivity (Lemma \ref{lem:commutativitytransitive}), all of these mutations commute with each other.}

\begin{lemma}
\label{lem:hierarchicalcommutativity3}
Given a commutativity index built over a sequence of composite mutations $\mathbb M$, for any composite mutation $\mut \in \collbar$ of bounded path length and complexity, the highest log index $i$ for which $\mathbb M_i \sqcup \readset(\mut) \neq \emptyset$ can be computed in $O(\readset(\mut))$ time
\end{lemma}

\proof{The index $i$ is the maximum of the $start$ or $child$ values of all paths $\phi \sqsubseteq \readset(\mut)$}

\begin{lemma}
\label{lem:hierarchicalcommutativity4}
Given a commutativity index built over a sequence of composite mutations $\mathbb M$, for any composite mutation $\mut \in \collbar$ of bounded path length and complexity, the highest log index $i$ for which $\mut \sqcup \readset(\mathbb M_i) \neq \emptyset$ can be computed in constant time.
\end{lemma}

\proof{The index $i$ is the maximum of the $read$ values of all paths $\phi \sqsubseteq \readset(\mut)$}

\begin{theorem}
\label{thm:commutativityindex}
For a log $\mathbb M$ of mutations $\mut \in \collbar$ of bounded path length and complexity, the amortized computational complexity of maintaining a list of mutations $\mathbb M_i$ for which $\oraclecomm(\mathbb M_i, \mathbb M_j)$ for all $j \geq i$, is $O(|\readset(\mut)|)$.
\end{theorem}

\proof{By Lemmas \ref{lem:hierarchicalcommutativity1}, \ref{lem:hierarchicalcommutativity2-2}, \ref{lem:hierarchicalcommutativity3}, and \ref{lem:hierarchicalcommutativity4}, we have the necessary conditions of commutativity with the last entry of the log.  These lemmas produce a maximum index that we refer to as the commutativity {\em threshold}.  

The deletion maps can be used in a similar manner to identify the set of target lists for paths appearing in one of these ancestor-aware (inclusive-)intersections.  There will be:\\ $O(|\readset(\mut)|)$ such target lists. 

Any mutation on one of these lists with an index equal to or preceding the commutativity threshold does not commute with the tail.  These entries are deleted from the target lists and from the set of mutations that can be commuted to the tail of the log.  The cost of each step in the iteration from the lowest index in the target list to the threshold index can be allocated to the cost of inserting the corresponding mutations into the log.}

\smallskip

Using Theorem \ref{thm:commutativityindex}, we can incrementally maintain a candidate set of mutations that can be correctly merged with the tail of the log in $O(|\readset(\mut)|)$ amortized time.  Although testing for recoverability requires linear time in the number of correct rewrite mutations available, a cost-based heuristic approach can be used to trim this list of mutations further.  These cost-based heuristics are beyond the scope of this paper and relegated to future work.


% LocalWords:  metadata subsumption bool unsubsumed datastructure bi
% LocalWords:  iff resp index's idempotence mutation's


==> motivation.tex <==
%\section{Laasie}
%\label{sec:motivation}
%\subsection{Roadmap}
%
%In this paper, we present BarQL, a language for querying and updating application state.  BarQL operates over a hierarchical datatype.  
%
%
%
%
%a state update language called BarQL.  
%
%
%We define a set of rules for 
%
%
%
%
%\begin{enumerate}
%
%\item hierarchical model based on key/value maps, with goal for
%supporting distributed systems naturally
%
%\item high and low/level semantic definition
%
%\item primitives for reasoning about log relevant operations in arbitrary language
%
%\item extension hierarchical data model
%
%\end{enumerate}

